A unified framework of fully distributed adaptive output time-varying formation control for linear multi-agent systems: an observer viewpoint

This paper presents a unified framework of time-varying formation (TVF) design for general linear multi-agent systems (MAS) based on an observer viewpoint from undirected to directed topology, from stabilization to tracking and from a leader without input to a one with bounded input. The followers can form a TVF shape which is specified by piecewise continuously differential vectors. The leader's trajectory, which is available to only a subset of followers, is also time-varying. For the undirected formation tracking and directed formation stabilization cases, only the relative output measurements of neighbors are required to design control protocols; for the directed formation tracking case, the agents need to be introspective (i.e. agents have partial knowledge of their own states) and the output measurements are required. Furthermore, considering the real applications, the leader with bounded input case is studied. One main contribution of this paper is that fully distributed adaptive output protocols, which require no global information of communication topology and do not need the absolute or relative state information, are proposed to solve the TVF control problem. Numerical simulations including an application to nonholonomic mobile vehicles are provided to verify the theoretical results.

==> ms <==
\begin{thebibliography}{43}
\expandafter\ifx\csname natexlab\endcsname\relax\def\natexlab#1{#1}\fi
\providecommand{\bibinfo}[2]{#2}
\ifx\xfnm\relax \def\xfnm[#1]{\unskip,\space#1}\fi
%Type = Article
\bibitem[{Olfati-Saber and Murray(2004)}]{olfati-saber_consensus_2004}
\bibinfo{author}{R.~Olfati-Saber}, \bibinfo{author}{R.~M. Murray},
\newblock \bibinfo{title}{Consensus problems in networks of agents with
  switching topology and time-delays},
\newblock \bibinfo{journal}{IEEE Transactions on Automatic Control}
  \bibinfo{volume}{49} (\bibinfo{year}{2004}) \bibinfo{pages}{1520--1533}.
%Type = Article
\bibitem[{Ren and Beard(2005)}]{ren_consensus_2005}
\bibinfo{author}{W.~Ren}, \bibinfo{author}{R.~W. Beard},
\newblock \bibinfo{title}{Consensus seeking in multiagent systems under
  dynamically changing interaction topologies},
\newblock \bibinfo{journal}{IEEE Transactions on Automatic Control}
  \bibinfo{volume}{50} (\bibinfo{year}{2005}) \bibinfo{pages}{655--661}.
%Type = Article
\bibitem[{Yu et~al.(2017)Yu, Wang, Cheng, Yu, and Wen}]{yu_second-order_2017}
\bibinfo{author}{W.~Yu}, \bibinfo{author}{H.~Wang}, \bibinfo{author}{F.~Cheng},
  \bibinfo{author}{X.~Yu}, \bibinfo{author}{G.~Wen},
\newblock \bibinfo{title}{Second-{Order} {Consensus} in {Multiagent} {Systems}
  via {Distributed} {Sliding} {Mode} {Control}},
\newblock \bibinfo{journal}{IEEE Transactions on Cybernetics}
  \bibinfo{volume}{47} (\bibinfo{year}{2017}) \bibinfo{pages}{1872--1881}.
%Type = Article
\bibitem[{Ji et~al.(2008)Ji, Ferrari-Trecate, Egerstedt, and
  Buffa}]{ji_containment_2008}
\bibinfo{author}{M.~Ji}, \bibinfo{author}{G.~Ferrari-Trecate},
  \bibinfo{author}{M.~Egerstedt}, \bibinfo{author}{A.~Buffa},
\newblock \bibinfo{title}{Containment {Control} in {Mobile} {Networks}},
\newblock \bibinfo{journal}{IEEE Transactions on Automatic Control}
  \bibinfo{volume}{53} (\bibinfo{year}{2008}) \bibinfo{pages}{1972--1975}.
%Type = Article
\bibitem[{Cheng et~al.(2016)Cheng, Wang, Ren, Hou, and
  Tan}]{cheng_containment_2016}
\bibinfo{author}{L.~Cheng}, \bibinfo{author}{Y.~Wang},
  \bibinfo{author}{W.~Ren}, \bibinfo{author}{Z.~G. Hou},
  \bibinfo{author}{M.~Tan},
\newblock \bibinfo{title}{Containment {Control} of {Multiagent} {Systems}
  {With} {Dynamic} {Leaders} {Based} on a $pi^{\textrm{n}}$ -{Type}
  {Approach}},
\newblock \bibinfo{journal}{IEEE Transactions on Cybernetics}
  \bibinfo{volume}{46} (\bibinfo{year}{2016}) \bibinfo{pages}{3004--3017}.
%Type = Article
\bibitem[{Fax and Murray(2004)}]{fax_information_2004}
\bibinfo{author}{J.~A. Fax}, \bibinfo{author}{R.~M. Murray},
\newblock \bibinfo{title}{Information flow and cooperative control of vehicle
  formations},
\newblock \bibinfo{journal}{IEEE Transactions on Automatic Control}
  \bibinfo{volume}{49} (\bibinfo{year}{2004}) \bibinfo{pages}{1465--1476}.
%Type = Article
\bibitem[{Tanner et~al.(2004)Tanner, Pappas, and
  Kumar}]{tanner_leader--formation_2004}
\bibinfo{author}{H.~G. Tanner}, \bibinfo{author}{G.~J. Pappas},
  \bibinfo{author}{V.~Kumar},
\newblock \bibinfo{title}{Leader-to-formation stability},
\newblock \bibinfo{journal}{IEEE Transactions on Robotics and Automation}
  \bibinfo{volume}{20} (\bibinfo{year}{2004}) \bibinfo{pages}{443--455}.
%Type = Article
\bibitem[{Dong and Hu(2016)}]{dong_time-varying_2016-1}
\bibinfo{author}{X.~Dong}, \bibinfo{author}{G.~Hu},
\newblock \bibinfo{title}{Time-varying formation control for general linear
  multi-agent systems with switching directed topologies},
\newblock \bibinfo{journal}{Automatica} \bibinfo{volume}{73}
  (\bibinfo{year}{2016}) \bibinfo{pages}{47--55}.
%Type = Article
\bibitem[{Wang and Xin(2013)}]{wang_integrated_2013}
\bibinfo{author}{J.~Wang}, \bibinfo{author}{M.~Xin},
\newblock \bibinfo{title}{Integrated {Optimal} {Formation} {Control} of
  {Multiple} {Unmanned} {Aerial} {Vehicles}},
\newblock \bibinfo{journal}{IEEE Transactions on Control Systems Technology}
  \bibinfo{volume}{21} (\bibinfo{year}{2013}) \bibinfo{pages}{1731--1744}.
%Type = Article
\bibitem[{Ghommam et~al.(2016)Ghommam, Luque-Vega, Castillo-Toledo, and
  Saad}]{ghommam_three-dimensional_2016}
\bibinfo{author}{J.~Ghommam}, \bibinfo{author}{L.~F. Luque-Vega},
  \bibinfo{author}{B.~Castillo-Toledo}, \bibinfo{author}{M.~Saad},
\newblock \bibinfo{title}{Three-dimensional distributed tracking control for
  multiple quadrotor helicopters},
\newblock \bibinfo{journal}{Journal of the Franklin Institute}
  \bibinfo{volume}{353} (\bibinfo{year}{2016}) \bibinfo{pages}{2344--2372}.
%Type = Article
\bibitem[{Antonelli et~al.(2014)Antonelli, Arrichiello, Caccavale, and
  Marino}]{antonelli_decentralized_2014}
\bibinfo{author}{G.~Antonelli}, \bibinfo{author}{F.~Arrichiello},
  \bibinfo{author}{F.~Caccavale}, \bibinfo{author}{A.~Marino},
\newblock \bibinfo{title}{Decentralized time-varying formation control for
  multi-robot systems},
\newblock \bibinfo{journal}{The Int'l Journal of Robotics Research}
  \bibinfo{volume}{33} (\bibinfo{year}{2014}) \bibinfo{pages}{1029--1043}.
%Type = Article
\bibitem[{Liu and Jiang(2013)}]{liu_distributed_2013}
\bibinfo{author}{T.~Liu}, \bibinfo{author}{Z.-P. Jiang},
\newblock \bibinfo{title}{Distributed formation control of nonholonomic mobile
  robots without global position measurements},
\newblock \bibinfo{journal}{Automatica} \bibinfo{volume}{49}
  (\bibinfo{year}{2013}) \bibinfo{pages}{592--600}.
%Type = Article
\bibitem[{Sakurama(2016)}]{sakurama_multi-robot_2016}
\bibinfo{author}{K.~Sakurama},
\newblock \bibinfo{title}{Multi-robot {Formation} {Control} over {Distance}
  {Sensor} {Network}},
\newblock \bibinfo{journal}{IFAC-PapersOnLine} \bibinfo{volume}{49}
  (\bibinfo{year}{2016}) \bibinfo{pages}{198--203}.
%Type = Article
\bibitem[{Peng et~al.(2013)Peng, Wen, Rahmani, and
  Yu}]{peng_leaderfollower_2013}
\bibinfo{author}{Z.~Peng}, \bibinfo{author}{G.~Wen},
  \bibinfo{author}{A.~Rahmani}, \bibinfo{author}{Y.~Yu},
\newblock \bibinfo{title}{Leader–follower formation control of nonholonomic
  mobile robots based on a bioinspired neurodynamic based approach},
\newblock \bibinfo{journal}{Robotics and Autonomous Systems}
  \bibinfo{volume}{61} (\bibinfo{year}{2013}) \bibinfo{pages}{988--996}.
%Type = Article
\bibitem[{Zhang and Liu(2016)}]{zhang_cooperative_2016}
\bibinfo{author}{M.~Zhang}, \bibinfo{author}{H.~H.~T. Liu},
\newblock \bibinfo{title}{Cooperative {Tracking} a {Moving} {Target} {Using}
  {Multiple} {Fixed}-wing {UAVs}},
\newblock \bibinfo{journal}{J Intell Robot Syst} \bibinfo{volume}{81}
  (\bibinfo{year}{2016}) \bibinfo{pages}{505--529}.
%Type = Article
\bibitem[{Nigam et~al.(2012)Nigam, Bieniawski, Kroo, and
  Vian}]{nigam_control_2012}
\bibinfo{author}{N.~Nigam}, \bibinfo{author}{S.~Bieniawski},
  \bibinfo{author}{I.~Kroo}, \bibinfo{author}{J.~Vian},
\newblock \bibinfo{title}{Control of {Multiple} {UAVs} for {Persistent}
  {Surveillance}: {Algorithm} and {Flight} {Test} {Results}},
\newblock \bibinfo{journal}{IEEE Transactions on Control Systems Technology}
  \bibinfo{volume}{20} (\bibinfo{year}{2012}) \bibinfo{pages}{1236--1251}.
%Type = Article
\bibitem[{Lewis and Tan(1997)}]{lewis_high_1997}
\bibinfo{author}{M.~A. Lewis}, \bibinfo{author}{K.-H. Tan},
\newblock \bibinfo{title}{High {Precision} {Formation} {Control} of {Mobile}
  {Robots} {Using} {Virtual} {Structures}},
\newblock \bibinfo{journal}{Autonomous Robots} \bibinfo{volume}{4}
  (\bibinfo{year}{1997}) \bibinfo{pages}{387--403}.
%Type = Article
\bibitem[{Das et~al.(2002)Das, Fierro, Kumar, Ostrowski, Spletzer, and
  Taylor}]{das_vision-based_2002}
\bibinfo{author}{A.~K. Das}, \bibinfo{author}{R.~Fierro},
  \bibinfo{author}{V.~Kumar}, \bibinfo{author}{J.~P. Ostrowski},
  \bibinfo{author}{J.~Spletzer}, \bibinfo{author}{C.~J. Taylor},
\newblock \bibinfo{title}{A vision-based formation control framework},
\newblock \bibinfo{journal}{IEEE Transactions on Robotics and Automation}
  \bibinfo{volume}{18} (\bibinfo{year}{2002}) \bibinfo{pages}{813--825}.
%Type = Article
\bibitem[{Balch and Arkin(1998)}]{balch_behavior-based_1998}
\bibinfo{author}{T.~Balch}, \bibinfo{author}{R.~C. Arkin},
\newblock \bibinfo{title}{Behavior-based formation control for multirobot
  teams},
\newblock \bibinfo{journal}{IEEE Transactions on Robotics and Automation}
  \bibinfo{volume}{14} (\bibinfo{year}{1998}) \bibinfo{pages}{926--939}.
%Type = Inproceedings
\bibitem[{Tanner(2004)}]{tanner_controllability_2004}
\bibinfo{author}{H.~G. Tanner},
\newblock \bibinfo{title}{On the controllability of nearest neighbor
  interconnections},
\newblock in: \bibinfo{booktitle}{Decision and {Control}, 2004. {CDC}. 43rd
  {IEEE} {Conference} on}, volume~\bibinfo{volume}{3},
  \bibinfo{publisher}{IEEE}, \bibinfo{year}{2004}, pp.
  \bibinfo{pages}{2467--2472}.
%Type = Article
\bibitem[{Peymani et~al.(2014)Peymani, Grip, Saberi, Wang, and
  Fossen}]{peymani_almost_2014}
\bibinfo{author}{E.~Peymani}, \bibinfo{author}{H.~F. Grip},
  \bibinfo{author}{A.~Saberi}, \bibinfo{author}{X.~Wang},
  \bibinfo{author}{T.~I. Fossen},
\newblock \bibinfo{title}{$ \mathcal{H}_{\infty} $ almost output
  synchronization for heterogeneous networks of introspective agents under
  external disturbances},
\newblock \bibinfo{journal}{Automatica} \bibinfo{volume}{50}
  (\bibinfo{year}{2014}) \bibinfo{pages}{1026--1036}.
%Type = Article
\bibitem[{Oh et~al.(2015)Oh, Park, and Ahn}]{oh_survey_2015}
\bibinfo{author}{K.-K. Oh}, \bibinfo{author}{M.-C. Park},
  \bibinfo{author}{H.-S. Ahn},
\newblock \bibinfo{title}{A survey of multi-agent formation control},
\newblock \bibinfo{journal}{Automatica} \bibinfo{volume}{53}
  (\bibinfo{year}{2015}) \bibinfo{pages}{424--440}.
%Type = Article
\bibitem[{Dong et~al.(2016)Dong, Li, Ren, and Zhong}]{dong_output_2016}
\bibinfo{author}{X.~Dong}, \bibinfo{author}{Q.~Li}, \bibinfo{author}{Z.~Ren},
  \bibinfo{author}{Y.~Zhong},
\newblock \bibinfo{title}{Output formation-containment analysis and design for
  general linear time-invariant multi-agent systems},
\newblock \bibinfo{journal}{Journal of the Franklin Institute}
  \bibinfo{volume}{353} (\bibinfo{year}{2016}) \bibinfo{pages}{322--344}.
%Type = Article
\bibitem[{Rahimi et~al.(2014)Rahimi, Abdollahi, and
  Naqshi}]{rahimi_time-varying_2014}
\bibinfo{author}{R.~Rahimi}, \bibinfo{author}{F.~Abdollahi},
  \bibinfo{author}{K.~Naqshi},
\newblock \bibinfo{title}{Time-varying formation control of a collaborative
  heterogeneous multi agent system},
\newblock \bibinfo{journal}{Robotics and Autonomous Systems}
  \bibinfo{volume}{62} (\bibinfo{year}{2014}) \bibinfo{pages}{1799--1805}.
%Type = Article
\bibitem[{Dong et~al.(2016)Dong, Xiang, Han, Li, and
  Ren}]{dong_distributed_2016}
\bibinfo{author}{X.~Dong}, \bibinfo{author}{J.~Xiang},
  \bibinfo{author}{L.~Han}, \bibinfo{author}{Q.~Li}, \bibinfo{author}{Z.~Ren},
\newblock \bibinfo{title}{Distributed {Time}-{Varying} {Formation} {Tracking}
  {Analysis} and {Design} for {Second}-{Order} {Multi}-{Agent} {Systems}},
\newblock \bibinfo{journal}{J Intell Robot Syst}  (\bibinfo{year}{2016})
  \bibinfo{pages}{1--13}.
%Type = Article
\bibitem[{Wang et~al.(2017)Wang, Dong, Li, and Ren}]{wang2017distributed}
\bibinfo{author}{R.~Wang}, \bibinfo{author}{X.~Dong}, \bibinfo{author}{Q.~Li},
  \bibinfo{author}{Z.~Ren},
\newblock \bibinfo{title}{Distributed time-varying formation control for linear
  swarm systems with switching topologies using an adaptive output-feedback
  approach},
\newblock \bibinfo{journal}{IEEE Transactions on Systems, Man, and Cybernetics:
  Systems}  (\bibinfo{year}{2017}).
%Type = Article
\bibitem[{Jadbabaie et~al.(2003)Jadbabaie, Lin, and
  Morse}]{jadbabaie_coordination_2003}
\bibinfo{author}{A.~Jadbabaie}, \bibinfo{author}{J.~Lin},
  \bibinfo{author}{A.~S. Morse},
\newblock \bibinfo{title}{Coordination of groups of mobile autonomous agents
  using nearest neighbor rules},
\newblock \bibinfo{journal}{IEEE Transactions on Automatic Control}
  \bibinfo{volume}{48} (\bibinfo{year}{2003}) \bibinfo{pages}{988--1001}.
%Type = Article
\bibitem[{Ren(2007)}]{ren_consensus_2007}
\bibinfo{author}{W.~Ren},
\newblock \bibinfo{title}{Consensus strategies for cooperative control of
  vehicle formations},
\newblock \bibinfo{journal}{IET Control Theory \& Applications}
  \bibinfo{volume}{1} (\bibinfo{year}{2007}) \bibinfo{pages}{505--512}.
%Type = Article
\bibitem[{Li et~al.(2011)Li, Liu, Lin, and Ren}]{li_consensus_2011}
\bibinfo{author}{Z.~Li}, \bibinfo{author}{X.~Liu}, \bibinfo{author}{P.~Lin},
  \bibinfo{author}{W.~Ren},
\newblock \bibinfo{title}{Consensus of linear multi-agent systems with
  reduced-order observer-based protocols},
\newblock \bibinfo{journal}{Systems \& Control Letters} \bibinfo{volume}{60}
  (\bibinfo{year}{2011}) \bibinfo{pages}{510--516}.
%Type = Article
\bibitem[{Cao et~al.(2013)Cao, Yu, Ren, and Chen}]{cao_overview_2013}
\bibinfo{author}{Y.~Cao}, \bibinfo{author}{W.~Yu}, \bibinfo{author}{W.~Ren},
  \bibinfo{author}{G.~Chen},
\newblock \bibinfo{title}{An {Overview} of {Recent} {Progress} in the {Study}
  of {Distributed} {Multi}-{Agent} {Coordination}},
\newblock \bibinfo{journal}{IEEE Transactions on Industrial Informatics}
  \bibinfo{volume}{9} (\bibinfo{year}{2013}) \bibinfo{pages}{427--438}.
%Type = Inproceedings
\bibitem[{Jiang et~al.(2017)Jiang, Wen, Meng, and
  Rahmani}]{jiang2017distributed}
\bibinfo{author}{W.~Jiang}, \bibinfo{author}{G.~Wen},
  \bibinfo{author}{Y.~Meng}, \bibinfo{author}{A.~Rahmani},
\newblock \bibinfo{title}{Distributed adaptive time-varying formation tracking
  for linear multi-agent systems: A dynamic output approach},
\newblock in: \bibinfo{booktitle}{Control Conference (CCC), 2017 36th Chinese},
  \bibinfo{organization}{IEEE}, pp. \bibinfo{pages}{8571--8576}.
%Type = Book
\bibitem[{Godsil and Royle(2001)}]{godsil_algebraic_2001}
\bibinfo{author}{C.~Godsil}, \bibinfo{author}{G.~F. Royle},
  \bibinfo{title}{Algebraic {Graph} {Theory}}, \bibinfo{publisher}{Springer
  Science \& Business Media}, \bibinfo{address}{New York, NY, USA},
  \bibinfo{year}{2001}.
%Type = Book
\bibitem[{Qu(2009)}]{qu_cooperative_2009}
\bibinfo{author}{Z.~Qu}, \bibinfo{title}{Cooperative {Control} of {Dynamical}
  {Systems}: {Applications} to {Autonomous} {Vehicles}},
  \bibinfo{publisher}{Springer Science \& Business Media},
  \bibinfo{year}{2009}.
%Type = Inproceedings
\bibitem[{Mei et~al.(2014)Mei, Ren, and Chen}]{mei_consensus_2014}
\bibinfo{author}{J.~Mei}, \bibinfo{author}{W.~Ren}, \bibinfo{author}{J.~Chen},
\newblock \bibinfo{title}{Consensus of second-order heterogeneous multi-agent
  systems under a directed graph},
\newblock in: \bibinfo{booktitle}{2014 {American} {Control} {Conference}}, pp.
  \bibinfo{pages}{802--807}.
%Type = Book
\bibitem[{Bernstein(2009)}]{bernstein_matrix_2009}
\bibinfo{author}{D.~S. Bernstein}, \bibinfo{title}{Matrix {Mathematics}:
  {Theory}, {Facts}, and {Formulas}.}, \bibinfo{publisher}{Princeton University
  Press}, \bibinfo{year}{2009}.
%Type = Article
\bibitem[{Wen et~al.(2016)Wen, Zhao, Duan, Yu, and Chen}]{wen_containment_2016}
\bibinfo{author}{G.~Wen}, \bibinfo{author}{Y.~Zhao}, \bibinfo{author}{Z.~Duan},
  \bibinfo{author}{W.~Yu}, \bibinfo{author}{G.~Chen},
\newblock \bibinfo{title}{Containment of {Higher}-{Order} {Multi}-{Leader}
  {Multi}-{Agent} {Systems}: {A} {Dynamic} {Output} {Approach}},
\newblock \bibinfo{journal}{IEEE Transactions on Automatic Control}
  \bibinfo{volume}{61} (\bibinfo{year}{2016}) \bibinfo{pages}{1135--1140}.
%Type = Article
\bibitem[{Li et~al.(2013)Li, Ren, Liu, and Fu}]{li_consensus_2013}
\bibinfo{author}{Z.~Li}, \bibinfo{author}{W.~Ren}, \bibinfo{author}{X.~Liu},
  \bibinfo{author}{M.~Fu},
\newblock \bibinfo{title}{Consensus of {Multi}-{Agent} {Systems} {With}
  {General} {Linear} and {Lipschitz} {Nonlinear} {Dynamics} {Using}
  {Distributed} {Adaptive} {Protocols}},
\newblock \bibinfo{journal}{IEEE Transactions on Automatic Control}
  \bibinfo{volume}{58} (\bibinfo{year}{2013}) \bibinfo{pages}{1786--1791}.
%Type = Article
\bibitem[{Lv et~al.(2016)Lv, Li, Duan, and Feng}]{lv_novel_2016}
\bibinfo{author}{Y.~Lv}, \bibinfo{author}{Z.~Li}, \bibinfo{author}{Z.~Duan},
  \bibinfo{author}{G.~Feng},
\newblock \bibinfo{title}{Novel distributed robust adaptive consensus protocols
  for linear multi-agent systems with directed graphs and external
  disturbances},
\newblock \bibinfo{journal}{International Journal of Control}
  \bibinfo{volume}{0} (\bibinfo{year}{2016}) \bibinfo{pages}{1--11}.
%Type = Article
\bibitem[{Hong et~al.(2006)Hong, Hu, and Gao}]{hong_tracking_2006}
\bibinfo{author}{Y.~Hong}, \bibinfo{author}{J.~Hu}, \bibinfo{author}{L.~Gao},
\newblock \bibinfo{title}{Tracking control for multi-agent consensus with an
  active leader and variable topology},
\newblock \bibinfo{journal}{Automatica} \bibinfo{volume}{42}
  (\bibinfo{year}{2006}) \bibinfo{pages}{1177--1182}.
%Type = Book
\bibitem[{Krstic et~al.(1995)Krstic, Kokotovic, and
  Kanellakopoulos}]{krstic_nonlinear_1995}
\bibinfo{author}{M.~Krstic}, \bibinfo{author}{P.~V. Kokotovic},
  \bibinfo{author}{I.~Kanellakopoulos}, \bibinfo{title}{Nonlinear and
  {Adaptive} {Control} {Design}}, \bibinfo{publisher}{John Wiley \& Sons,
  Inc.}, \bibinfo{address}{New York, NY, USA}, \bibinfo{edition}{1st} edition,
  \bibinfo{year}{1995}.
%Type = Article
\bibitem[{Khalil(1996)}]{khalil1996noninear}
\bibinfo{author}{H.~K. Khalil},
\newblock \bibinfo{title}{Noninear systems},
\newblock \bibinfo{journal}{Prentice-Hall, New Jersey} \bibinfo{volume}{2}
  (\bibinfo{year}{1996}) \bibinfo{pages}{5--1}.
%Type = Article
\bibitem[{Lv et~al.(2015)Lv, Li, Duan, and Chen}]{lv_fully_2015}
\bibinfo{author}{Y.~Lv}, \bibinfo{author}{Z.~Li}, \bibinfo{author}{Z.~Duan},
  \bibinfo{author}{J.~Chen},
\newblock \bibinfo{title}{Fully {Distributed} {Adaptive} {Output} {Feedback}
  {Protocols} for {Linear} {Multi}-{Agent} {Systems} with {Directed} {Graphs}:
  {A} {Sequential} {Observer} {Design} {Approach}},
\newblock \bibinfo{journal}{arXiv:1511.01297 [cs]}  (\bibinfo{year}{2015}).
%Type = Article
\bibitem[{Lawton et~al.(2003)Lawton, Beard, and
  Young}]{lawton_decentralized_2003}
\bibinfo{author}{J.~R.~T. Lawton}, \bibinfo{author}{R.~W. Beard},
  \bibinfo{author}{B.~J. Young},
\newblock \bibinfo{title}{A decentralized approach to formation maneuvers},
\newblock \bibinfo{journal}{IEEE Transactions on Robotics and Automation}
  \bibinfo{volume}{19} (\bibinfo{year}{2003}) \bibinfo{pages}{933--941}.

\end{thebibliography}

